Topological Pressure for Locally Compact Metrizable Systems

It is widely known that when $X$ is compact Hausdorff, and when $T: X \to X$ and $f: X \to \mathbb{R}$ are continuous, \begin{equation*} P(T,f) = \sup_{\text{$\mu$: Radon probability}} \left( h_\mu(T) + \int f\, \mathrm{d}\mu \right), \end{equation*} where $P(T,f)$ is the "topological pressure" and $h_\mu(T)$ is the measure theoretic entropy of $T$ with respect to $\mu$. This result is known as "variational principle". We generalize the concept of "topological pressure" for the case where $X$ is a separable locally compact metric space. Our definitions are quite similar to those used in the compact case. Our main result is the validity of the "variational principle".

==> principio_variacional_para_pressao/definitions.tex <==
\RequirePackage{mathrsfs} % Font \mathscr

\theoremstyle{plain}

\newtheorem{theorem}{Theorem}[section]     %% @uncomment@NO_theorems_with_chapter_numbering@

\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{affirmation}{Claim}
\newenvironment{proofitemenv}
  {\par\noindent\vspace{10pt}\rule{1ex}{1ex}\hspace{2ex}} %TODO: clear left.
  {\par}
\newtheorem{case}{Case}
\newtheorem*{notation}{Notation}
\newtheorem{definition}[theorem]{Definition}

% Horrível: o estilo "definition" não é bom para definição e notação!
% Horrível: estilo "remark" é ruim para observações e exemplos!!
\theoremstyle{definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{obs}[theorem]{Remark}

\providecommand{\email}[1]{{#1}}


%Divides de proof into cases. (TODO: not good yet.)
\newlength{\affrule}
\providecommand{\subproof}[2]
{{
  \begin{quote}
    \begin{affirmation}
      {#1}
    \end{affirmation}

    \parindent .5cm %\parskip .2cm
    {#2}
  \end{quote}
  \vspace{10pt}
}}

\providecommand{\subcase}[2]
{{
  \vspace{10pt}
  \begin{case}
    {#1}
  \end{case}

  {#2}
}}

\providecommand{\proofitem}[2]
{{
  \vspace{15pt}
  \begin{proofitemenv}
    {#1}
  \end{proofitemenv}

  {#2}
}}


%Não sei se é o latex ou se sou eu, mas as "referências" não têm a cara certa!
\providecommand{\refeq}[1]{{(\ref{#1})}}
\providecommand{\refitem}[1]{{(\ref{#1})}}


% Commonly used sets.
\providecommand{\naturals}[0]{\mathbb{N}}
\providecommand{\integers}[0]{\mathbb{Z}}
\providecommand{\rationals}[0]{\mathbb{Q}}
\providecommand{\reals}[0]{\mathbb{R}}
\providecommand{\nonnegativereals}[0]{\mathbb{R^+}}
\providecommand{\complexes}[0]{\mathbb{C}}

\providecommand{\family}[1]{{\mathscr{#1}}}
\providecommand{\parts}[1]{{\family{P}\left(#1\right)}}

% Special symbols.
\providecommand{\suchthat}[0]{{\thickspace | \thickspace}}
\providecommand{\cardinality}[1]{{\# #1}}

% Brackets.
\newcommand{\threebracket}[5]{{\left #1 \vphantom{{#2}^N}\vphantom{{#4}^N}{#2} \, \right #3 \left. \vphantom{{#2}^N}\vphantom{{#4}^N}{#4} \right #5}}

\providecommand{\setsuchthat}[2]{{\threebracket{\{}{#1}{|\:}{#2}{\}}}}
\providecommand{\set}[1]{{\left \{ {#1} \right \}}}
\providecommand{\abs}[1]{{\left\lvert#1\right\rvert}}
\providecommand{\norm}[2][]{{\left\lVert{#2}\right\rVert_{#1}}}

\newcommand{\integral}[3][]{{\int_{#1} {#2}\, \mathrm{d}{#3}}}
\newcommand{\conditionalexpectation}[2]{{E \threebracket{(}{#1}{|}{#2}{)}}}
\newcommand{\qtp}[1]{{[{#1}-\qtpop]}}

% Operator names.
\DeclareMathOperator{\identity}{id}
\DeclareMathOperator{\interiorop}{int}
\DeclareMathOperator{\closureop}{cl}
\DeclareMathOperator{\supportop}{supp}
\DeclareMathOperator{\qtpop}{qtp}

\DeclareMathOperator{\eigenspace}{eig}
\DeclareMathOperator{\expbase}{e}


% Functions
\newcommand{\function}[3]{{#1: #2 \to #3}}
\newcommand{\functionmaps}[3]{{#1: #2 \mapsto #3}}
\newcommand{\functionarray}[5]{{\begin{array}[t]{lrcl}
                                  #1:& #2 &\to     &#3 \\
                                     & #4 &\mapsto &#5
                                \end{array}}}

% Operations
\newcommand{\closure}[1]{{\overline{#1}}}
%\newcommand{\closure}[1]{{\closureop \left({#1}\right)}}
%\newcommand{\interior}[1]{{\mathring{#1}}}
\newcommand{\interior}[1]{\interiorop \left({#1}\right)}
\newcommand{\complementset}[1]{{#1}^{c}}
\newcommand{\powerset}[1]{{\mathscr{P}({#1})}}
\newcommand{\indicator}[1]{{I_{#1}}}
\newcommand{\support}[1]{{\supportop \left( {#1} \right)}}


\newcommand{\ball}[3][]{{B_{#1}\left({#3}; {#2}\right)}}
\newcommand{\balls}[2]{{\family{B}_{#1}\left({#2}\right)}}


\newcommand{\covercardinality}[2][]{{N_{#1}\left({#2}\right)}}
\newcommand{\separatedcardinality}[3]{{s\left({#1}, {#2}, {#3}\right)}}

\newcommand{\radonprobabilities}[1]{{\mathcal{P}\left({#1}\right)}}
\newcommand{\invariantradonprobabilities}[2]{{\mathcal{P}_{{#1}}\left({#2}\right)}}
\newcommand{\radonmeasures}[1]{{\mathcal{M}\left({#1}\right)}}
\newcommand{\invariantradonmeasures}[2]{{\mathcal{M}_{{#1}}\left({#2}\right)}}
\newcommand{\radonball}[1]{{\mathcal{B}\left({#1}\right)}}
\newcommand{\invariantradonball}[2]{{\mathcal{B}_{{#1}}\left({#2}\right)}}

\newcommand{\dynamicalsystem}[2]{{\function{#2}{#1}{#1}}}

\newcommand{\borelsets}[0]{{\family{B}}}
\newcommand{\measurablesets}[1]{{\family{B}}}
\newcommand{\measurablespace}[1]{{\left({#1}, \measurablesets{#1}\right)}}
\newcommand{\probability}[1]{{\mu}}
\newcommand{\measure}[1]{{\mu}}
\newcommand{\probabilityspace}[1]{{\left({#1}, \measurablesets{#1}, \probability{#1}\right)}}
\newcommand{\measurespace}[1]{{\left({#1}, \measurablesets{#1}, \measure{#1}\right)}}


\newcommand{\partitionentropy}[2]{{H_{#1}\left({#2}\right)}}
\newcommand{\tpartitionentropy}[3]{{h_{#1}\left({#3}, {#2}\right)}}
\newcommand{\measureentropy}[2]{{h_{#1}\left({#2}\right)}}

\newcommand{\conditionalprobability}[3]{{{#1}\threebracket{(}{#3}{|}{#2}{)}}}
\newcommand{\conditionalpartitionentropy}[3]{{H_{#1}\threebracket{(}{#2}{|}{#3}{)}}}

%\newcommand{\topology}[1]{{\tau}}
%\newcommand{\topologicalspace}[1]{{\left({#1}, \topology{#1}\right)}}
\newcommand{\topologicalspace}[1]{{#1}}

\newcommand{\metricspace}[2]{{\left({#1}, {#2}\right)}}
\newcommand{\iteratedmetric}[2]{{{#1}_{#2}}}

\newcommand{\coverentropy}[1]{{H\left({#1}\right)}}
\newcommand{\tcoverentropy}[2]{{h\left({#2}, {#1}\right)}}

\newcommand{\topologicalentropy}[1]{{h\left({#1}\right)}}

\newcommand{\bowenentropy}[2]{{h_{#1}\left({#2}\right)}}
\newcommand{\dentropy}[2]{{h^{#1}\left({#2}\right)}}
\newcommand{\epsilonbowenentropy}[4]{{h_{#1}\left({#2}, {#3}, {#4}\right)}}
\newcommand{\epsilondentropy}[3]{{h^{#1}\left({#2}, {#3}\right)}}


\newcommand{\continuousfunctions}[1]{{C\left(#1\right)}}
\newcommand{\compactsuportfunctions}[1]{{C_c\left(#1\right)}}
\newcommand{\vanishingatinfinityfunctions}[1]{{C_0\left(#1\right)}}


\newcommand{\compactification}[1]{{\widetilde{#1}}}
\newcommand{\onepointcompactification}[1]{{{#1}^*}}

